Teachable Reality: Prototyping Tangible Augmented Reality with Everyday Objects by Leveraging Interactive Machine Teaching

This paper introduces Teachable Reality, an augmented reality (AR) prototyping tool for creating interactive tangible AR applications with arbitrary everyday objects. Teachable Reality leverages vision-based interactive machine teaching (e.g., Teachable Machine), which captures real-world interactions for AR prototyping. It identifies the user-defined tangible and gestural interactions using an on-demand computer vision model. Based on this, the user can easily create functional AR prototypes without programming, enabled by a trigger-action authoring interface. Therefore, our approach allows the flexibility, customizability, and generalizability of tangible AR applications that can address the limitation of current marker-based approaches. We explore the design space and demonstrate various AR prototypes, which include tangible and deformable interfaces, context-aware assistants, and body-driven AR applications. The results of our user study and expert interviews confirm that our approach can lower the barrier to creating functional AR prototypes while also allowing flexible and general-purpose prototyping experiences.

==> rebuttal.tex <==
We are grateful for the feedback and delighted that reviewers found our work to be novel, highly significant, well-motivated, and easy to follow with well-made and creative example figures and videos. We address the concerns raised by reviewers:

TECHNICAL NOVELTY (1AC, 2AC)
We acknowledge 2AC's concern about the technical novelty. We would like to emphasize that our article makes a "systems contributions". In particular, in line with the "Novel functionality known technique" quadrant in the systems contribution space [A], R3 identifies that "While the technique used is not novel in itself, the combination of an existing technique with a streamlined prototyping workflow makes it a novel contribution." 

Furthermore, an expert participant described our approach as more than just Teachable Machine + AR, highlighting 
1) its deployability, 2) in situ AR authoring, and 3) the ability to animate virtual content when transitioning between states. To the best of our knowledge, these features make our approach a valuable contribution to the field of tangible AR prototyping, and we hope the reviewers will consider these aspects in their evaluation.

[A] Kumar, Nebeling, and Laput. "A Note from the UIST 2021 PC Chairs" [https://medium.com/acm-uist/a-note-from-the-uist-2021-pc-chairs-6a30df14f33b]

DESIGN SPACE - Supported Modalities & Applications (1AC, 2AC, R2)
In response to the reviewers' concern, we have added more information on how we came up with the design space to provide more context and rationale for this categorization. Through the process, we first investigated and collected existing research on tangible interfaces, then identified common input and output elements for tangible AR applications. Therefore, we have added representative examples for each element in the Figure. Since this is not a systematic search, we do not claim that this design space is exhaustive, but we believe it provides a clearer understanding of the common elements of input and output for tangible AR applications, not only about what each element but also about why they need and how they are used in the prior applications. 

Furthermore, as suggested by the reviewers, we have also merged the Application section with the Supported Modalities section. We hope these changes address the reviewers' concerns and provide a clearer understanding of our work.

USER STUDY (1AC, R2)
We also acknowledge the need for more depth in the insights presented in our usability study and have added more comments from the participants to provide a richer discourse. The usability study was designed to get objective measures with optional subjective questions, whereas we sought open-ended discussion and deep insights about our interaction with the experts. Though we agree with R2's suggestion to study how the system enables the two user groups differently will be an interesting insight, we don't comment on it as both studies had different parameters and metrics. 

We acknowledge 2AC's concern that Unity + Vuforia could be considered a baseline for some limited features. In fact, we considered other systems, such as RealityComposer or Aero, as potential baselines but found that these existing systems were insufficient to investigate how users can incorporate various tangible inputs. Additionally, in our usability study, participants often did not have experience in AR development, whereas Unity still expects basic knowledge of 3D game programming and app development. Therefore, we conducted a qualitative comparison with the existing tools through expert interviews rather than a user study. 

IMPLEMENTATION (1AC, R2)
We want to clarify that the applications shown in our figures were created using our system, and as suggested by R2, we are also happy to release the system as open-source. Note that some features, such as surface detection and anchoring, may not be available due to the requirement of a paid subscription to 8th Wall's private APIs. We plan to prepare both simplified and full versions when releasing the code. 

LIMITATIONS (1AC, R1)
We move the limitations mentioned by the experts to the limitations section. By reorganizing, we highlight the opportunities it creates for future work.

Suggestions incorporated into the draft. 
Contribution (R3) - 1 & 3 Contribution have been merged
Related works (R3) - Change in Terminology and rephrasing for more clarity, corrected incorrect statement that Rapido was not functional
Preliminary Study (R3) - Explicitly mentioned the methods used to analyze the studies in Section 3
Implementation (2AC) - Moved before the Design Space section
Other Minor changes pointed out by reviewers
